A Graphical Approach to Progress for Structured Communication in Web Services

We investigate a graphical representation of session invocation interdependency in order to prove progress for the pi-calculus with sessions under the usual session typing discipline. We show that those processes whose associated dependency graph is acyclic can be brought to reduce. We call such processes transparent processes. Additionally, we prove that for well-typed processes where services contain no free names, such acyclicity is preserved by the reduction semantics. Our results encompass programs (processes containing neither free nor restricted session channels) and higher-order sessions (delegation). Furthermore, we give examples suggesting that transparent processes constitute a large enough class of processes with progress to have applications in modern session-based programming languages for web services.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{Bliudze, Bruni, Grohmann, Silva (Eds.):\\Third Interaction and Concurrency Experience (ICE 2010)\\
EPTCS 38, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.38.4}{10.4204/EPTCS.38.4}}
\pdfoutput=1

